DexVLA: Vision-Language Model with Plug-In Diffusion Expert for General Robot Control

Enabling robots to perform diverse tasks across varied environments is a central challenge in robot learning. While vision-language-action (VLA) models have shown promise for generalizable robot skills, realizing their full potential requires addressing limitations in action representation and efficient training. Current VLA models often focus on scaling the vision-language model (VLM) component, while the action space representation remains a critical bottleneck. This paper introduces DexVLA, a novel framework designed to enhance the efficiency and generalization capabilities of VLAs for complex, long-horizon tasks across diverse robot embodiments. DexVLA features a novel diffusion-based action expert, scaled to one billion parameters, designed for cross-embodiment learning. A novel embodiment curriculum learning strategy facilitates efficient training: (1) pre-training the diffusion expert that is separable from the VLA on cross-embodiment data, (2) aligning the VLA model to specific embodiments, and (3) post-training for rapid adaptation to new tasks. We conduct comprehensive experiments across multiple embodiments, including single-arm, bimanual, and dexterous hand, demonstrating DexVLA's adaptability to challenging tasks without task-specific adaptation, its ability to learn dexterous skills on novel embodiments with limited data, and its capacity to complete complex, long-horizon tasks using only direct language prompting, such as laundry folding. In all settings, our method demonstrates superior performance compared to state-of-the-art models like Octo, OpenVLA, and Diffusion Policy.

==> sec/1_introduction_old.tex <==
\vspace{-0.4cm}
\section{Introduction}
%Imitation learning has been shown to be an effective way to teach robots a wide range of motor skills, such as grasping, legged locomotion, dexterous manipulation, humanoid loco-manipulation, and mobile manipulation. Visual imitation learning, which takes high-dimensional visual observations such as images or depth maps, eases the need for task-specific state estimation and thus gains the popularity.

%However, the generality of visual imitation learning comes at a cost of vast demonstration

%Replicating human-like behavior in robots is an immense challenge, requiring seamless integration of visual perception, language comprehension, and dexterous skill execution. Achieving versatility—defined as the ability to solve a variety of tasks across diverse environments, while adapting to language commands, environmental constraints, and unexpected disruptions—is an even greater challenge. Imitation learning, particularly through vision-language-action (VLA) models~\cite{black2024pi_0, rt-2, kim24openvla, wen2024tinyvla, ecot, wen2024diffusionvla, pertsch2025fast}, has demonstrated remarkable potential in enabling generalizable skills across diverse real-world scenarios. However, their reliance on massive human-generated datasets and imbalanced architectures limits scalability and real-world applicability.


Enabling robots to perform diverse tasks across varied environments is a central challenge in robotics. Achieving versatility—the ability to solve a variety of tasks across diverse environments, while adapting to language commands, environmental constraints, and unexpected disruptions—is even more demanding. Imitation learning, particularly through vision-language-action (VLA) models (e.g., \cite{black2024pi_0, rt-2, kim24openvla}), has shown promise in enabling generalizable skills. 


However, realizing the vision of omnipotent robot foundation models faces persistent challenges. Two key bottlenecks hinder progress: 2) Data scarcity: State-of-the-art models, like OpenVLA~\cite{openvla}/Octo~\cite{octo}, rely on massive datasets like the Open-X Embodiment dataset (4,000 hours)~\cite{o2023open-x} or even larger corpora like the 10,000-hour dataset used by ~\cite{[pi0}. Collecting such data through human demonstrations is extremely costly and labor-intensive. (2) Architectural imbalance: current VLA models often prioritize scaling the vision-language model (VLM) component, i.e., OpenVLA uses 7B VLM and $\pi_{0}$ uses 3B VLM. Despite its enhanced visual and multimodal understanding through internet-scale data pretraining, the VLM component remains disconnected from the embodied, sensorimotor context of robotic action.

This paper introduces Vision-Language-Action models using Diffusion Expert for X-embodiement, namely Dex-VLA, a novel framework designed to enhance the efficiency and generalization capabilities of VLA for complex, long-horizon tasks across diverse robot embodiments. We achieve this through two key innovations:


\textbf{1. Billion-Parameter Diffusion Expert}: Recognizing the limitations of conventional action experts, particularly in handling cross-embodiment data, we propose a new diffusion-based action expert. The diffusion expert utilizes a multi-head architecture, with each head corresponding to a specific embodiment, enabling effective learning across diverse morphologies.  Furthermore, we scale the model size of the diffusion expert to one billion parameters, a substantial increase from the conventional multi-million parameter scale. This scaling significantly enhances the model's capacity to learn intricate motor skills and control policies from diverse and extensive data.

\textbf{2. Embodied Curriculum Learning}: A three-stage training strategy that progressively learns harder tasks. This is conceptually similar to how human learn, which starts with simple tasks, and then gradually introduces complexity to avoid overwhelming the learner.

\textbf{Stage 1:} The \textbf{cross-embodiment pre-training} stage is to teach model learning basic motor skills that are low-level and embodiment-agnostic skills. We pre-train exclusively the diffusion expert using cross-embodiment data. This stage does not involve vision-language models.

%This pre-training significantly reduces computational overhead compared to conventional VLA training, which typically involves pre-training the entire model.

\textbf{Stage 2:} The \textbf{embodiment-specific alignment} is a stage that analogy to ''adapt to your body". Specifically, it bridges abstract vision-language representations to the physical constraints of a specific robot. Remarkably, this stage alone enables the model to complete a variety of tasks, such as shirt folding and bin picking on in-domain objects.

%We bridge the semantic gap between vision-language representations and embodiment-specific action spaces by training the complete VLA model on data from a single embodiment. Remarkably, this stage alone enables the model to successfully complete a variety of tasks, such as shirt folding on a mobile bimanual robot.
\textbf{Stage 3:} The \textbf{task-specific adaptation} aims to make the robot master complex tasks. These tasks include completing long-horizon tasks and generalizing to novel objects. 

%This curriculum structure directly addresses the “embodiment disconnect” in prior VLAs: by first learning universal physical principles (Stage 1) before specializing to morphology-specific control (Stage 2), the model avoids overfitting to narrow datasets while retaining the ability to generalize across hardware platforms.


%Three key bottlenecks hinder progress: (1) Data dependency: State-of-the-art VLAs like OpenVLA [cite] and $\pi_{0}$ require thousands of hours of costly human demonstrations to pre-training (from Open X-Embodiement,4k–10k hours [cite]), creating scalability barriers. (2) Architectural imbalance: Pre-trained VLMs operate in abstract representation spaces, poorly capturing the sensorimotor grounding required for physical interaction. However, state-of-the-art approaches leverage VLM from 3B to 7B parameters, the action spaces remain underdeveloped (typically 0–300M parameters), misaligning resource allocation with embodied control demands. 


%We present VLA-Dexpert, a framework that rethinks VLA architecture and training to address these limitations. By rebalancing model capacity toward embodiment-aware action spaces and introducing data-efficient learning strategies, our approach enables robust, generalizable robot control for diverse complex and long-horizon tasks on different embodiments. We achieve
%this through two key innovations: 
%1. Billion-Parameter Diffusion Expert: A multi-head architecture scales action-space modeling to 1B parameters, enabling cross-embodiment skill transfer (e.g., bimanual to mobile robots) while reducing compute costs by 30\% via decoupled pre-training.



%long-horizon tasks (e.g., laundry folding) without auxiliary policy frameworks.


%Developing omnipotent robot foundation models that can generalize across diverse tasks and environments is a critical yet challenging goal in robotics. However, realizing this vision is fraught with several persistent challenges. Primarily, the performance of these models is intrinsically linked to the quality and quantity of training data. State-of-the-art models, such as OpenVLA~\cite{openvla}/Octo~\cite{octo}, are pre-trained on the Open-X Embodiment dataset, encompassing 4,000 hours of robotic teleoperation data~\cite{o2023open-x}, while $\pi_{0}$~\cite{[pi0} leverages an even larger corpus of 10,000 hours. Collecting these datasets through human demonstrations is labor-intensive and costly. This reliance on vast, manually curated data creates a significant bottleneck, necessitating the development of strategies for more efficient data utilization. Furthermore, the current trend of training vision-language models is to focus on making vision-language model parts to learn the action space of robots. These models, although pre-trained on massive internet-scale datasets to enhance their visual and linguistic understanding, are still largely disconnected from the physical world. VLMs primarily operate in a space of abstract representations, rather than in the embodied, sensorimotor context in which robots function. Therefore, heavily relying on VLM to train data from embodied robots may be suboptimal. Recent works have scaled the VLM component of Vision-Language Action (VLA) models from 2B to 72B parameters~\cite{diffusionvla}, yet the benefits of scaling the VLM alone appear marginal. In contrast, the action space component of VLA models remains relatively small, ranging from 15M to 300M parameters. This observation suggests the need to re-evaluate the architectural design of VLA models, shifting the focus away from solely scaling the VLM component and exploring novel training strategies for holistic model enhancement.


%This paper introduces VLA-Dexpert, a novel framework designed to enhance the efficiency and generalization capabilities of Visuomotor Language Agents (VLAs) for complex, long-horizon tasks across diverse robot embodiments.  We achieve this through two key innovations:


%\noindent
%\textbf{1. Diffusion Expert:} Recognizing the limitations of conventional action experts in handling cross-embodiment data and large-scale datasets, we propose a new diffusion-based action expert. This expert utilizes a multi-head architecture, with each head corresponding to a specific embodiment, enabling effective learning across diverse morphologies.  Furthermore, we scale the model size of the diffusion expert to one billion parameters, a substantial increase from the conventional multi-million parameter scale. This scaling significantly enhances the model's capacity to learn intricate motor skills and control policies from diverse and extensive data.


%\noindent
%\textbf{2. Three-Stage Training Strategy:} To efficiently train this enhanced architecture, we introduce a novel three-stage training strategy. 
%\\
%\textbf{Stage 1:} We pre-train exclusively the diffusion expert using cross-embodiment data. This pre-training significantly reduces computational overhead compared to conventional VLA training, which typically involves pre-training the entire model.
%\\
%\textbf{Stage 2:} We bridge the semantic gap between vision-language representations and embodiment-specific action spaces by training the complete VLA model on data from a single embodiment. Remarkably, this stage alone enables the model to successfully complete a variety of tasks, such as shirt folding on mobile bimanual robot.
%\\
%\textbf{Stage 3:} To further enhance performance on complex, long-horizon tasks, we introduce a post-training stage focused on high-quality, task-specific data. This lightweight adaptation process also allows VLA-Dexpert to be rapidly tailored to new tasks and environments.

As up to this step, the model are able to learn from diverse behavior coming from different robots and learn progressively to enable a certain embodiment to stable skill to deal with more complex tasks. Nevertheless, for very long-horizon tasks, such as folding 
We evaluate Dex-VLA across a variety of embodiments, including single-arm, bimanual, dexterous hand, and mobile bimanual robots, and demonstrate its effectiveness on a diverse set of tasks. Notably, our approach successfully completes challenging tasks like \textbf{laundry folding} using \textbf{only direct prompting}, eliminating the need for high-level policy frameworks like $\pi_0$~\cite{black2024pi_0} that uses SayCan~\cite{ahn2022can}. We believe VLA-Dexpert represents a promising direction for architectural design and training paradigms in end-to-end general robot control.

The contributions of our work consist a novel neural architecture for robot policy learning and an associated training strategy that maximize the potential of this framework. While our framework shares similarities with concepts in vision-language models, its application to robotic learning, particularly for end-to-end imitation learning on complex and dexterous tasks at this level, has not been shown. We evaluate our method across multiple embodiments under various conditions, including zero-shot generalization, learning dexterous skills on novel embodiments, and following complex, long-horizon instructions.


%To address the aforementioned challenges, this paper introduces VLA-Dexpert, a framework designed to facilitate generalizable visuomotor policy to learn efficiently on complex, long-horizon tasks on diverse robots. VLA-Dexpert achieves significant advancements through two perspectives. First, we design a new action expert, namely the diffusion expert. Because the model is trained with cross-embodiment data, our diffusion expert uses a multi-head architecture, each head corresponds to one embodiment. Furthermore, since the model is accepting with diverse large scale data, using small diffusion expert can be sub-optimal, which does not have so large capacity to learn the action. Therefore, we scale the model size of diffusion experts, from conventionally multi-million parameters to one billion parameters. This substantial scaling of the diffusion expert significantly enhances the model's capacity to learn complex motor skills and control policies.

%Secondly, we propose a novel three-stage training strategy that learns the generalizable visuomotor policy efficiently and effectively. At stage 1, in a departure from conventional VLA training paradigms that necessitate the pretraining of the entire model, we pre-train exclusively the diffusion expert with cross-embodiment data. Given the significantly reduced parameter count of the action expert compared to the complete VLA model, this approach drastically reduces the computational overhead associated with pre-training. The stage 2 aims to effectively bridge the semantic gap between vision-language representations and specific embodiment action spaces. This stage if trained the entirely model with only one embodiment data. Notably, after training at this stage, the model are able to complete most tasks, such as shirt folding. Finally, for more complex and long-horizon task, the model need to do post-training, which trains particularly on high-quality data for specific task. This stage can also be regarded as a lightweight adaptation process, enabling VLA-Dexpert to be swiftly tailored to new tasks and environments. 






%Our diffusion expert uses multi-head architecture to 


%it strategically scales the action expert module to 1 billion parameters in Transformer architecture, compared to previous methods that use multi-million diffusion model parameters. This substantial scaling of the action expert, a critical component for generating effective actions, significantly enhances the model's capacity to learn complex motor skills and control policies. 



%in a departure from conventional VLA training paradigms that necessitate the pretraining of the entire model, i.e., $\pi_{0}$ and OpenVLA, our proposed VLA-Dexpert focuses exclusively on pre-training the action expert. Given the significantly reduced parameter count of the action expert compared to the complete VLA model, this approach drastically reduces the computational overhead associated with pre-training. 


%Following the pre-training phase, VLA-Dexpert employs a refined two-stage fine-tuning strategy. The initial embodiment alignment stage, conceptually analogous to the alignment process in VLMs, aims to effectively bridge the semantic gap between vision-language representations and action outputs. This alignment facilitates rapid adaptation of the pre-trained action expert to downstream tasks. Subsequently, a post-training stage further refines the action expert's performance on specific tasks, optimizing its capabilities for target applications. The two-stage fine-tuning can be regarded as a lightweight adaptation process, enabling XXXX-VLA to be swiftly tailored to new tasks and environments.




%a based on VLM pre-training and flow
%atching, and an empirical investigation of pre-training/posttraining recipes for such robot foundation models.



%In summary, our contributions are four-fold:
%5\begin{itemize}
 %   \item We propose a new paradigm of vision-language-action models, with a new design of diffusion expert and a novel training strategy that effectively learns generalizable and versatile robot control. 
  %  \item We evaluate our proposed VLA-Dexpert in a broad range of embodiments, including a single-arm, bimanual, robot with a dexterous hand, and a mobile bimanual robot, showing the universality applicability of VLAction.
  %  \item We demonstrate that our method can complete challenging tasks like shirt folding \textbf{without post-training}, finishing complex tasks like laundry folding with \textbf{direct prompting}, and  learning \textbf{new dexterous skills} with only 50 demonstrations.  
    %\item We demonstrate that with less than 50 hours of data for pre-training, our method can conduct a broad range of real-world tasks, from long-horizontal tasks (laundry folding) to dexterous tasks (i.e., bussing table with novel objects). 
%\end{itemize}

==> sec/8_acknolwedgement.tex <==
We would like to thank Yanjie Ze for valuable discussion. We also like to thank Xiaoyu Liu, Zhongyi Zhou, Chengmeng Li, Peiting Zhao for data collection. 
